Protein Multimer Structure Prediction via Prompt Learning

Understanding the 3D structures of protein multimers is crucial, as they play a vital role in regulating various cellular processes. It has been empirically confirmed that the multimer structure prediction~(MSP) can be well handled in a step-wise assembly fashion using provided dimer structures and predicted protein-protein interactions~(PPIs). However, due to the biological gap in the formation of dimers and larger multimers, directly applying PPI prediction techniques can often cause a \textit{poor generalization} to the MSP task. To address this challenge, we aim to extend the PPI knowledge to multimers of different scales~(i.e., chain numbers). Specifically, we propose \textbf{\textsc{PromptMSP}}, a pre-training and \textbf{Prompt} tuning framework for \textbf{M}ultimer \textbf{S}tructure \textbf{P}rediction. First, we tailor the source and target tasks for effective PPI knowledge learning and efficient inference, respectively. We design PPI-inspired prompt learning to narrow the gaps of two task formats and generalize the PPI knowledge to multimers of different scales. We provide a meta-learning strategy to learn a reliable initialization of the prompt model, enabling our prompting framework to effectively adapt to limited data for large-scale multimers. Empirically, we achieve both significant accuracy (RMSD and TM-Score) and efficiency improvements compared to advanced MSP models. The code, data and checkpoints are released at \url{https://github.com/zqgao22/PromptMSP}.

==> table/table-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\setlength{\tabcolsep}{1.5pt}
\renewcommand\arraystretch{0.8}
\centering
\caption{\textbf{Multimer structure prediction results.} Baseline methods are evaluated on the test set of $3\leq N \leq 10$ by using two types of dimers. For each dimer type and metric, the best method is \textbf{bold} and the second best is \underline{underlined}. $\dag$ represents the reassembly version of baselines.}
\vspace{0.7em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
\multirow{2}{*}{\textbf{\scalebox{1.3}{Methods}}} & \multicolumn{4}{c|}{\textbf{\texttt{\scalebox{1.2}{GT Dimer}}}}                                   & \multicolumn{4}{c}{\textbf{\texttt{\scalebox{1.2}{AFM Dimer}}}}                                     \\ \cmidrule(l){2-9} 
                                  & \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Median)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Median)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Median)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Median)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{Multi-LZerD}         & 59.19 & 62.70 & 0.35 & 0.33 & 59.19 & 62.70 & 0.35 & 0.33 \\
\multicolumn{1}{l|}{$\text{Multi-LZerD}^{\dag}$}         & 57.48 & 58.01 & 0.37 & 0.36 & 60.77 & 59.72 & 0.36 & 0.32 \\ \midrule
\multicolumn{1}{l|}{RL-MLZerD}       & 57.70 & 60.16 & 0.36 & 0.36 & 57.70 & 60.16 & 0.36 & 0.36 \\
\multicolumn{1}{l|}{$\text{RL-MLZerD}^{\dag}$}         & 54.13 & 52.72 & 0.39 & 0.37 & 57.37 & 57.60 & 0.33 & 0.38 \\ \midrule
\multicolumn{1}{l|}{AFM}                & 31.17 & 32.02 & 0.46 & 0.48 & 31.17 & 32.02 & 0.46 & 0.48 \\ 
\multicolumn{1}{l|}{$\text{AFM}^{\dag}$}                & \underline{27.70} & 29.91 & 0.50 & \underline{0.56} & \underline{30.05} & \underline{30.70} & \underline{0.47} & \underline{0.50} \\  \midrule
\multicolumn{1}{l|}{MoLPC}              & 29.56 & \underline{28.98} & \underline{0.55} &  \underline{0.56} & 34.21 & 36.54 & 0.42 & 0.45 \\
\multicolumn{1}{l|}{\textbf{\textsc{PromptMSP}}} & \textbf{22.09} & \textbf{23.15} & \textbf{0.65} & \textbf{0.67} & \textbf{27.77} & \textbf{29.50} & \textbf{0.51} & \textbf{0.55} \\ \midrule
\multicolumn{1}{l|}{Ours vs. MoLPC}                          & 25.27\% & 20.11\% & 18.18\% & 19.64\% & 18.82\% & 19.27\% & 21.43\% & 22.22\% \\ \bottomrule
\end{tabular}%
}\label{table:main}
\end{table}

==> table/table-10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\setlength{\tabcolsep}{1.5pt}
\renewcommand\arraystretch{0.8}
\centering
\caption{\textcolor{blue}{\textbf{Multimer structure prediction results under the \textbf{\texttt{HDock Dimer}} and \textbf{\texttt{ESMFold Dimer}} settings.} Baseline methods are evaluated on the test set of $3\leq N \leq 10$ by using two types of dimers. For each dimer type and metric, the best method is \textbf{bold} and the second best is \underline{underlined}. $\dag$ represents the reassembly version of baselines.}}
\vspace{0.7em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
\multirow{2}{*}{\textbf{\scalebox{1.3}{Methods}}} & \multicolumn{4}{c|}{\textbf{\texttt{\scalebox{1.2}{HDock Dimer}}}}                                   & \multicolumn{4}{c}{\textbf{\texttt{\scalebox{1.2}{ESMFold Dimer}}}}                                     \\ \cmidrule(l){2-9} 
                                  & \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Median)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Median)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RMSD$\downarrow$\\ (Median)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Mean)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TM-Score$\uparrow$\\ (Median)\end{tabular} \\ \midrule
\multicolumn{1}{l|}{Multi-LZerD}         & 59.19 & 62.70 & 0.35 & 0.33 & 59.19 & 62.70 & 0.35 & 0.33 \\
\multicolumn{1}{l|}{$\text{Multi-LZerD}^{\dag}$}         & 55.71 & 56.33 & 0.38 & 0.39 & 57.61 & 58.52 & 0.36 & 0.35 \\ \midrule
\multicolumn{1}{l|}{RL-MLZerD}       & 57.70 & 60.16 & 0.36 & 0.36 & 57.70 & 60.16 & 0.36 & 0.36 \\
\multicolumn{1}{l|}{$\text{RL-MLZerD}^{\dag}$}         & 55.27 & 54.26 & 0.37 & 0.38 & 56.03 & 58.29 & 0.36 & 0.40 \\ \midrule
\multicolumn{1}{l|}{AFM}                & 31.17 & 32.02 & 0.46 & 0.48 & \underline{31.17} & \underline{32.02} & \underline{0.46} & \underline{0.48} \\ 
\multicolumn{1}{l|}{$\text{AFM}^{\dag}$}                & \underline{29.17} & 31.78 & 0.48 & 0.46 & 32.44 & 33.98 & 0.45 & 0.43 \\  \midrule
\multicolumn{1}{l|}{MoLPC}              & 30.76 & \underline{31.00} & \underline{0.50} &  \underline{0.53} & 40.73 & 40.94 & 0.39 & 0.40 \\
\multicolumn{1}{l|}{\textbf{\textsc{PromptMSP}}} & \textbf{25.39} & \textbf{26.81} & \textbf{0.54} & \textbf{0.58} & \textbf{28.34} & \textbf{28.54} & \textbf{0.49} & \textbf{0.50}  \\ \bottomrule
\end{tabular}%
}\label{table:main}
\end{table}

==> table/table-2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{11}{c}{\textbf{Chain numbers N}}                                       \\ \cmidrule(l){2-12} 
                                  & 3 & 4 & 5 & 6-10 & 11-15 & 16-20 & 21-25 & 26-30 & 31-35 & 36-40 & \textgreater{}40 \\ \midrule
Multi-zerd                        &   &   &   &      &       &       &       &       &       &       &                  \\
RL-multizerd                      &   &   &   &      &       &       &       &       &       &       &                  \\
AF-multimer                       &   &   &   &      &       &       &       &       &       &       &                  \\
ESMFold                           &   &   &   &      &       &       &       &       &       &       &                  \\
MoLPC                             &   &   &   &      &       &       &       &       &       &       &                  \\
\textbf{DiffDP}                   & \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}  &  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$} & \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}  &   \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}   &     \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}  &   \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}    &   \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}    &   \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}    &  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}     &  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}     &  \colorbox[HTML]{CBCEFB}{$0.12_{\pm 0.99}$}                \\ \bottomrule
\end{tabular}%
}
\end{table}

==> table/table-3.tex <==
\begin{wraptable}{r}{6.1cm}
\vspace{1.2em}
\caption{Comparsion of inference time~(hr).}\label{table:time}
\centering
\setlength{\tabcolsep}{1.5pt}
\renewcommand\arraystretch{1.5}
\resizebox{0.43\textwidth}{!}{%
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|ccccc@{}}
\toprule
\textbf{Methods} & Multi-LZerD & RL-MLZerD & AFM & MoLPC & \textbf{Ours} \\ \midrule
    $3\leq N \leq 10$           &    $1.357$         &   $1.591$        &  $0.640$   &    $0.159$   &  $0.003$    \\ \midrule
  $11\leq N \leq 30$            &     -        &        -   &  -   &     $1.374$  &  $0.012$    \\ \bottomrule
\end{tabular}%
}
}
\vspace{-2em}
\end{wraptable}



==> table/table-5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h!]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Hyperparameters}                                            & \textbf{Values}                                            \\ \midrule
Embedding function dimension~(input)                                   & 13                                                \\
GIN layer number $K$                                  & 5                                               \\
Dimension of MLP in Eq.~\ref{eq7}     & 13, 64,64,128,128                                            \\
Dimension of $\phi$ in Eq.~\ref{eq1} & 128, 1                                            \\

Dropout rate                                               & 0.2                                               \\
Number of attention head                                   & 4                                                 \\

Task batch size                                                 & 20                                                 \\
Initial learning rates $\alpha,\eta$                                             & $1\times10^{-2},1\times 10^{-4}$ \\
Optimizer                                                  & Adam                                              \\ \bottomrule
\end{tabular}%
}
\vspace{1em}\caption{\footnotesize Hyperparameter choices of \textsc{PromptMSP}.}
\end{table}

==> table/table-6.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccccc|c@{}}
\toprule
$N$              & 3    & 4   & 5   & 6   & 7   & 8   & 9   & 10  & 11-15 & 16-20 & 21-25 & 26-30 & Sum  \\ \midrule
\textbf{Train} & 1325 & 942 & 981 & 856 & 952 & 875 & 543 & 421 & 267   & 198   & 135   & 66    & 7561 \\
\textbf{Valid} & 265  & 188 & 196 & 171 & 191 & 175 & 109 & 84  & 53    & 40    & 27    & 14    & 1513 \\
\textbf{Test}  & 20   & 20  & 20  & 20  & 20  & 20  & 20  & 20  & 25    & 25    & 25    & 25    & 260  \\ \bottomrule
\end{tabular}%
}\caption{The dataset statistic of PDB-M.}\label{table:dataset}
\end{table}

==> table/table-7.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\textbf{Thresholds} & 1998-1-1 & 2003-1-1 & 2008-1-1 & 2013-1-1 & 2018-1-1 \\ \midrule
\textbf{Train}      & 4578     & 5345     & 7081     & 7942     & 8340     \\
\textbf{Test}       & 4766     & 3999     & 2263     & 1402     & 1004     \\ \bottomrule
\end{tabular}%
}\caption{Data split statistic with date thresholds.}\label{table:date}
\end{table}

==> table/tmp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
                                  & \multicolumn{3}{c}{GT dimer} & \multicolumn{3}{c}{AF-mm dimer} & \multicolumn{3}{c}{ESMFold dimer} \\ \cmidrule(l){2-10} 
\multirow{-2}{*}{\textbf{Methods}} &
  RMSD (\uparrow) &
  TM-Score (\uparrow) &
  \multicolumn{1}{c|}{DockQ (\uparrow)} &
  RMSD (\uparrow) &
  TM-Score (\uparrow) &
  \multicolumn{1}{c|}{DockQ (\uparrow)} &
  RMSD (\uparrow) &
  TM-Score (\uparrow) &
  DockQ (\uparrow) \\ \midrule
\multicolumn{1}{l|}{Multi-zerd}   &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{RL-multizerd} &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{AF-multimer}  &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{ESMFold}      &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{MoLPC}        &   &  & \multicolumn{1}{c|}{} &    &   & \multicolumn{1}{c|}{}  &           &           &           \\
\multicolumn{1}{l|}{\textbf{DiffDP}} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{DAE8FC} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{CBCEFB} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CBCEFB}} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{CBCEFB} &
  \cellcolor[HTML]{CBCEFB} \\ \midrule
Ours vs. MoLPC &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}%
}
\end{table}
